Biased tracer reconstruction with halo mass information

Plenty of crucial information about our Universe is encoded in the cosmic large-scale structure (LSS). However, the extractions of these information are usually hindered by the nonlinearities of the LSS, which can be largely alleviated by various techniques known as the reconstruction. In realistic applications, the efficiencies of these methods are always degraded by many limiting factors, a quite important one being the shot noise induced by the finite number density of biased matter tracers (i.e., luminous galaxies or dark matter halos) in observations. In this work, we explore the gains of biased tracer reconstruction achieved from halo mass information, which can suppress shot noise component and dramatically improves the cross-correlation between tracer field and dark matter. To this end, we first closely study the clustering biases and the stochasticity properties of halo fields with various number densities under different weighting schemes, i.e., the uniform, mass and optimal weightings. Then, we apply the biased tracer reconstruction method to these different weighted halo fields and investigate how linear bias and observational mass scatter affect the reconstruction performance. Our results demonstrate that halo masses are critical information for significantly improving the performance of biased tracer reconstruction, indicating a great application potential for substantially promoting the precision of cosmological measurements [especially for baryon acoustic oscillations (BAO)] in the ambitious on-going and future galaxy surveys.

==> biased tracer reconstruction/defn_apj.tex <==
%-*-LaTeX-*-
% Copied from gmorris
% Note that some of these call others, eg \kmps uses \km.

% journals
%\newcommand{\apj}{ApJ}
%\newcommand{\mnras}{MNRAS}
%\newcommand{\nat}{Nat}
%\newcommand{\physrevB}{Phys. Rev. B}
%\newcommand{\araa}{ARA\&A}                % "Ann. Rev. Astron. Astrophys."
%\newcommand{\aap}{A\&A}                   % "Astron. Astrophys."
%\newcommand{\aaps}{A\&AS}                 % "Astron. Astrophys. Suppl. Ser."
%\newcommand{\aj}{AJ}                      % "Astron. J."
%\newcommand{\apjs}{ApJS}                  % "Astrophys. J. Suppl. Ser."
%\newcommand{\pasp}{PASP}                  % "Publ. Astron. Soc. Pac."
%\newcommand{\apjl}{ApJ}                   % letter at ApJ
%\newcommand{\pasj}{PASJ}
%\newcommand{\gca}{Geochim. Cosmochim. Acta}
%\newcommand{\physrep}{Phys. Rep.}
%\newcommand{\aapr}{A\&A Rev.}
%\newcommand{\ssr}{Space Sci. Rev.}
%\newcommand{\na}{New Astron.}
%\newcommand{\nar}{NewA Rev.}
%\newcommand{\jgr}{J. Geophys. Res.}

% Length
\newcommand{\Mpc}{\rm\; Mpc}
\newcommand{\kpc}{\rm\; kpc}
\newcommand{\pc}{\rm\; pc}
\newcommand{\km}{\rm\; km}
\newcommand{\m}{\rm\; m}
\newcommand{\cm}{\rm\; cm}
\newcommand{\mum}{\hbox{$\rm\; \mu m\,$}}
\newcommand{\pix}{\rm\; pixel}
%
\newcommand{\cmps}{\hbox{$\cm\s^{-1}\,$}}
\newcommand{\cmpssq}{\hbox{$\cm\s^{-2}\,$}}
\newcommand{\cmsq}{\hbox{$\cm^2\,$}}
\newcommand{\cmcu}{\hbox{$\cm^3\,$}}
\newcommand{\pcmcuK}{\hbox{$\cm^{-3}\K\,$}}
\newcommand{\ppix}{\hbox{$\pix^{-1}\,$}}
\newcommand{\ppixsq}{\hbox{$\pix^{-2}\,$}}
\newcommand{\kpcsq}{\hbox{$\kpc^{2}\,$}}
% Length


% Time
\newcommand{\hr}{\rm\; hr}
\newcommand{\yr}{\rm\; yr}
\newcommand{\Gyr}{\rm\; Gyr}
\newcommand{\Myr}{\rm\; Myr}
\newcommand{\s}{\rm\; s}
\newcommand{\ms}{\rm\; ms}
\newcommand{\ks}{\rm\; ks}
\newcommand{\mus}{\hbox{$\rm\; \mu s\,$}}
% Time


% Frequency
\newcommand{\GHz}{\rm\; GHz}
\newcommand{\MHz}{\rm\; MHz}
\newcommand{\kHz}{\rm\; kHz}
\newcommand{\Hz}{\rm\; Hz}
% Frequency


% Temperature
\newcommand{\K}{\rm\; K}
% Temperature


% Pressure
\newcommand{\Kpcmc}{\hbox{$\K\cm^{-3}\,$}}
\newcommand{\keVpcmcu}{\hbox{$\keV\cm^{-3}\,$}}
% Pressure


% Mass
\newcommand{\g}{\rm\; g}
%
\newcommand{\gpcm}{\hbox{$\g\cm^{-3}\,$}}
\newcommand{\gpcmps}{\hbox{$\g\cm^{-3}\s^{-1}\,$}}
\newcommand{\gps}{\hbox{$\g\s^{-1}\,$}}
\newcommand{\gpcmsq}{\hbox{$\g\cm^{-2}\,$}}
%
\newcommand{\Msun}{\hbox{$\rm\thinspace M_{\odot}$}}
\newcommand{\Msunpkpc}{\hbox{$\Msun\kpc^{-1}\,$}}
\newcommand{\Msunpcukpc}{\hbox{$\Msun\kpc^{-3}\,$}}
\newcommand{\Msunpsqpc}{\hbox{$\Msun\pc^{-2}\,$}}
\newcommand{\Msunpcupc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunppcpyr}{\hbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\newcommand{\Msunpyr}{\hbox{$\Msun\yr^{-1}\,$}}
\newcommand{\Msunpyrpsqkpc}{\hbox{$\Msunpyr\kpc^{-2}\,$}}
% Mass


% Energy
\newcommand{\MeV}{\rm\; MeV}
\newcommand{\keV}{\rm\; keV}
\newcommand{\eV}{\rm\; eV}
\newcommand{\erg}{\rm\; erg}
\newcommand{\Jy}{\rm\; Jy}
\newcommand{\mJy}{\rm\; mJy}
\newcommand{\W}{\rm\; W}
%
\newcommand{\ergcmcups}{\hbox{$\erg\cm^3\ps\,$}}
\newcommand{\ergpcmps}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergpcmsq}{\hbox{$\erg\cm^{-2}\,$}}
\newcommand{\ergpcmcu}{\hbox{$\erg\cm^{-3}\,$}}
\newcommand{\ergpcmsqps}{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
\newcommand{\ergpcmsqpspA}{\hbox{$\erg\cm^{-2}\s^{-1}$\AA$^{-1}\,$}}
\newcommand{\ergpcmsqpspsr}{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\newcommand{\ergpcmcups}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergps}{\hbox{$\erg\s^{-1}\,$}}
\newcommand{\ergpspHz}{\hbox{$\erg\s^{-1}\pHz\,$}}
\newcommand{\ergpspmp}{\hbox{$\erg\s^{-1}\Mpc^{-3}\,$}}
\newcommand{\ergpspkpc}{\hbox{$\erg\s^{-1}\kpc^{-1}\,$}}
%
\newcommand{\keVpcmsqpspsr}{\hbox{$\keV\cm^{-2}\s^{-1}\sr^{-1}\,$}}
%
\newcommand{\WpHzpsr}{\hbox{$\W\pHz\psr\,$}}
\newcommand{\WpHz}{\hbox{$\W\pHz\,$}}
%
\newcommand{\surbri}{\hbox{$\rm\thinspace photons\pcmsq\ps\pasecsq$}}
\newcommand{\expmapcorr}{\hbox{$\rm\thinspace photons\pcmsq\ps\ppix$}}
%
\newcommand{\Jykmps}{\hbox{$\Jy\km\s^{-1}\,$}}
\newcommand{\Jypbmkmps}{\hbox{$\Jy{\rm /beam}.{\rm km}\s^{-1}\,$}}
\newcommand{\mJypbm}{\hbox{$\mJy{\rm /beam}$}}
\newcommand{\Kkmps}{\hbox{$\K\km\s^{-1}\,$}}
% Energy


% Force
\newcommand{\dyn}{\rm\; dyn}
\newcommand{\dynpcmsq}{\hbox{$\dyn\cm^{-2}\,$}}
% Force


% Speed
\newcommand{\kmps}{\hbox{$\km\s^{-1}\,$}}
\newcommand{\kmpspmp}{\hbox{$\km\s^{-1}\Mpc{-1}\,$}}
\newcommand{\kmpspMpc}{\hbox{$\kmps\Mpc^{-1}\,$}}
% Speed


% Luminosity
\newcommand{\Lsun}{\hbox{$\rm\thinspace L_{\odot}$}}
\newcommand{\Lsunppc}{\hbox{$\Lsun\pc^{-3}\,$}}
% Luminosity


% Misc
\newcommand{\dex}{\rm\; dex}

\newcommand{\plawnorm}{\hbox{$\rm\thinspace photons\keV^{-1}\cm^{-2}\s^{-1}\,$}}
\newcommand{\Zsun}{\hbox{$\thinspace \mathrm{Z}_{\odot}$}}

\newcommand{\gauss}{\rm\; gauss}
\newcommand{\muG}{\hbox{$\rm\thinspace {\mu}\mathrm{G}$}}
%
\newcommand{\chisq}{\hbox{$\chi^2$}}
\newcommand{\delchi}{\hbox{$\Delta\chi$}}
%
\newcommand{\ph}{\rm\; ph}
% Misc

% Angles
\newcommand{\amin}{\rm\; arcmin}
\newcommand{\aminsq}{\hbox{$\amin^{2}\,$}}
\newcommand{\asec}{\rm\; arcsec}
\newcommand{\asecsq}{\hbox{$\asec^{2}\,$}}
\newcommand{\sr}{\rm\; sr}
\newcommand{\degword}{\rm\; deg}
\newcommand{\degsq}{\hbox{$\degword^2\,$}}
% Angles

% Emission measure
\newcommand{\emm}{\hbox{$\cm^{-5}\,$}}
\newcommand{\sqremm}{\hbox{$\cm^{-5/2}\,$}}
\newcommand{\empasecsq}{\hbox{$\emm\asec^{-2}\,$}}
\newcommand{\keVempasecsq}{\hbox{$\keV\emm\asec^{-2}\,$}}
\newcommand{\pseudoP}{\hbox{$\keV\sqremm\asec^{-2}\,$}}
% Emission measure

% Per something
\newcommand{\pcm}{\hbox{$\cm^{-1}\,$}}
\newcommand{\psqcm}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmsq}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmcu}{\hbox{$\cm^{-3}\,$}}
\newcommand{\pcmcus}{\hbox{$\pcmcu\s\,$}}
\newcommand{\pmpc}{\hbox{$\Mpc^{-1}\,$}}
\newcommand{\pmpccu}{\hbox{$\Mpc^{-3}\,$}}
\newcommand{\ps}{\hbox{$\s^{-1}\,$}}
\newcommand{\pHz}{\hbox{$\Hz^{-1}\,$}}
\newcommand{\pcmK}{\hbox{$\cm^{-3}\K$}}
\newcommand{\phpcmsqps}{\hbox{$\ph\cm^{-2}\s^{-1}\,$}}
\newcommand{\psr}{\hbox{$\sr^{-1}\,$}}
\newcommand{\pasecsq}{\hbox{$\asec^{-2}\,$}}
% Per something

\newcommand{\COtoH}{\hbox{$\psqcm(\K\kmps)^{-1}$}}

% Use times for maths fonts
% \DeclareSymbolFont{operators}   {OT1}{ptmcm}{m}{n}
% \DeclareSymbolFont{letters}     {OML}{ptmcm}{m}{it}
% \SetMathAlphabet{\mathbf}{normal}{\encodingdefault}{\rmdefault}{\bfdefault}{n}%
% \SetMathAlphabet{\mathsf}{normal}{\encodingdefault}{\sfdefault}{m}{n}%
% \SetMathAlphabet{\mathrm}{normal}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetSymbolFont{operators}{bold}{OT1}{ptmcm}{b}{n}
% \SetSymbolFont{letters}{bold}{OML}{ptmcm}{b}{it}
% \SetMathAlphabet{\mathbf}{bold}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetMathAlphabet{\mathsf}{bold}{\encodingdefault}{\sfdefault}{b}{n}%
% \SetMathAlphabet{\mathrm}{bold}{\encodingdefault}{\rmdefault}{b}{n}%

%\thinmuskip=2.5mu
%\medmuskip=3.5mu plus 1mu minus 1mu
%\thickmuskip=4.5mu plus 1.5mu minus 1mu
%\DeclareSymbolFont{symbols}     {OMS}{cmsy}{m}{n}
%\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
%\SetSymbolFont{symbols}{bold}{OMS}{cmsy}{b}{n}
%\SetSymbolFont{largesymbols}{bold}{OMX}{cmex}{m}{n}

